VLR-Bench: Multilingual Benchmark Dataset for Vision-Language Retrieval Augmented Generation

We propose the VLR-Bench, a visual question answering (VQA) benchmark for evaluating vision language models (VLMs) based on retrieval augmented generation (RAG). Unlike existing evaluation datasets for external knowledge-based VQA, the proposed VLR-Bench includes five input passages. This allows testing of the ability to determine which passage is useful for answering a given query, a capability lacking in previous research. In this context, we constructed a dataset of 32,000 automatically generated instruction-following examples, which we denote as VLR-IF. This dataset is specifically designed to enhance the RAG capabilities of VLMs by enabling them to learn how to generate appropriate answers based on input passages. We evaluated the validity of the proposed benchmark and training data and verified its performance using the state-of-the-art Llama3-based VLM, the Llava-Llama-3 model. The proposed VLR-Bench and VLR-IF datasets are publicly available online.

==> table/VLR_Bench_wh.tex <==
\begin{table}[h]
    \tiny
    \centering
    \begin{tabular}{l|rrr|r}
        \toprule
        & WRB & WDT & WP & Total \\
        \midrule
        what & 0 & 42 & 330 & 372 \\
        which & 0 & 82 & 0 & 82 \\
        how & 26 & 0 & 0 & 26 \\
        when & 14 & 0 & 0 & 14 \\
        who & 0 & 0 & 9 & 9 \\
        that & 0 & 7 & 0 & 7 \\
        where & 6 & 0 & 0 & 6 \\
        why & 2 & 0 & 0 & 2 \\
        \bottomrule
    \end{tabular}
    \caption{VLR-Bench의 instruction 의문사 분석}
    \label{table:vlr-bench-instruction}
\end{table}


==> table/chinese_eval_table.tex <==
\begin{table}[]
    \centering
    \tiny
    \begin{tabular}{lccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{5}{c}{Chinese}  \\
    \cmidrule(lr){2-6}               & MS     & R-1    & R-2    & R-L     & BLEU \\
    \midrule
    \textsc{LLaVA1.5(13B)}           & 4.4    & 2.8    & 0.9    & 2.8     & 0.0 \\
    \midrule
    \textsc{CHINESE-LLaVA}           & 29.2   & 20.4   & 6.6    & 20.3    & 0.0 \\
    \midrule
    \textsc{QWEN-VL-CHAT}            & 75.6   & 27.1   & 10.0    & 26.7    & 9.0  \\
    \textsc{QWEN-VL-CHAT+VLR-IF(Zh)} & 72.4   & 27.0   & 10.3    & 27.0    & 14.9  \\
    %\textsc{LLaVA1.5(13B)+Ours} & 50.8 & 27.3   & 27.2  & 1.2 \\
    \bottomrule
    \end{tabular}
    \label{tab:keyword_matching_ch}
    \caption{Keyword matching result chinese}
    
\end{table}



==> table/english_eval_table.tex <==
\begin{table}[]
    \centering
    \tiny
    \begin{tabular}{lccccc}
        \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{\vspace{-0.5em}Model}} & \multicolumn{5}{c}{English} \\
        \cmidrule(lr){2-6} 
                                   & MS & R-1 & R-2 & R-L & BLEU \\
        \midrule
        \textsc{BLIP-2}            & 50.0 & 36.0 & 19.9 & 33.0 & 4.9 \\
        \midrule
        \textsc{InstructBLIP}      & 32.0 & 44.6 & 26.7 & 38.1 & 11.2 \\
        \midrule
        %\textsc{LLaVA1.5 (7B)}     & 84.8 & 46.0   & 39.6 & 14.7  \\
        \textsc{LLaVA1.5 (13B)}    & 88.4 & 47.9 & 32.1  & 41.4 & 15.6  \\
        %\midrule
        %\textsc{Xtuner1.0}         & 84.0 & 47.0   & 41.1 & 13.8  \\
        \midrule
        \textsc{Xtuner1.1}         & 79.2 & 48.5 & 33.3  & 42.8 & 15.4  \\
        \textsc{Xtuner1.1+VLR-IF(En)}    & 85.6 & 60.4 & 42.0  & 54.1 & 26.8  \\
        \midrule
        \textsc{X-LLaVA}           & 80.4 & 54.3 & 35.8  & 47.2 & 20.2 \\
        \textsc{X-LLaVA+VLR-IF(En)}  & 82.4 & 57.7 & 37.9  & 50.5 & 24.3 \\
        %\textsc{X-LLaVA+Ours(Ko)}  & 78.7  & 59.1  & 52.1 & 24.8 \\
        \textsc{X-LLaVA+VLR-IF(En+Ko)} & 83.8 & 58.8 & 39.6 & 51.9 & 25.3  \\
        \midrule
        \textsc{Qwen-VL-Chat}           & 84.8 & 61.5 & 43.4 & 55.8 & 25.0 \\
        \midrule[0.8pt]
        \textsc{GPT-4o} & 85.6 & 74.2 & 57.9 & 69.5 & 41.9  \\
        \bottomrule
    \end{tabular}
    \caption{Keyword matching result english}
    \label{tab:keyword_matching_en}
\end{table}



==> table/keyword_matching.tex <==

\begin{table}[]
    \tiny
    \begin{tabular}{c|cccc|cccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{\vspace{-0.5em}Model}} & \multicolumn{4}{c|}{English} & \multicolumn{4}{c}{Korean} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
                               & MS & ROUGE-1 & ROUGE-L & BLEU & MS & ROUGE-1 & ROUGE-L & BLEU \\
    \midrule
    \textsc{BLIP-2}            & 50.0 & 36.0   & 33.0 & 4.9   & -   & -   & -  & - \\
    \midrule
    \textsc{InstructBLIP}      & 32.0 & 44.6   & 38.1   & 11.2 & -   & -   & - & - \\
    \midrule
    \textsc{LLaVA1.5 (7B)}     & 84.8 & 46.0   & 39.6 & 14.7  & 80.0 & 25.0 & 24.7 & 5.4 \\
    \textsc{LLaVA1.5 (13B)}    & 88.4 & 47.9   & 41.4 & 15.6  & 65.2   & 14.2  & 14.1 & 4.4 \\
    \midrule
    \textsc{Xtuner1.0}         & 84.0 & 47.0   & 41.1 & 13.8  & -   & -  & -   \\
    \midrule
    \textsc{Xtuner1.1}         & 79.2 & 48.5   & 42.8 & 15.4   & -   & -  & -   \\
    \textsc{Xtuner1.1+Ours}    & 85.6 & 60.4   & 54.1 & 26.8   & -  & -  & -  \\
    \midrule
    \textsc{KoLLaVA}           & -    & -      & -  &  -   & 66.0 & 20.6 & 20.5 & 4.1 \\       
    \midrule
    \textsc{X-LLaVA}           & 80.4 & 54.3   & 47.2 & 20.2  & 59.6 & 15.7 & 15.8 & 12.2 \\
    \textsc{X-LLaVA+Ours(En)}  & 82.4 & 57.7   & 50.5 & 24.3  & 62.8 & 25.9 & 25.8 & 13.3 \\
    \textsc{X-LLaVA+Ours(Ko)}  & 82.4 & 57.7   & 50.5 & 24.3  & 62.8 & 25.9 & 25.8 & 13.3 \\
    \textsc{X-LLaVA+Ours(En+Ko)}      & 82.8 & 58.8   & 51.9 & 25.3  & 62.4 & 25.2 & 25.2 & 12.2 \\       
    \bottomrule
    \end{tabular}
    \caption{Keyword matching result}
    \label{tab:keyword_matching_enxx}
\end{table}



==> table/korean_eval_table.tex <==
% \begin{table}[]
%     \tiny
%     \begin{tabular}{c|cccc}
%     \toprule
%     \multicolumn{1}{c|}{\multirow{2}{*}{\vspace{-0.5em}Model}} & \multicolumn{4}{c|}{English} & \multicolumn{4}{c}{Korean} \\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%                                & MS & ROUGE-1 & ROUGE-L & BLEU \\
%     \midrule
%     \textsc{LLaVA1.5 (7B)}     & 80.0 & 25.0 & 24.7 & 5.4 \\
%     \textsc{LLaVA1.5 (13B)}    & 65.2   & 14.2  & 14.1 & 4.4 \\
%     \midrule
%     \textsc{KoLLaVA}           & 66.0 & 20.6 & 20.5 & 4.1 \\       
%     \midrule
%     \textsc{X-LLaVA}           & 59.6 & 15.7 & 15.8 & 12.2 \\
%     \textsc{X-LLaVA+Ours(En)}  & 62.8 & 25.9 & 25.8 & 13.3 \\
%     \textsc{X-LLaVA+Ours(En+Ko)}      & 62.4 & 25.2 & 25.2 & 12.2 \\       
%     \bottomrule
%     \end{tabular}
%     \caption{Keyword matching result}
%     \label{tab:korean_eval_table}
% \end{table}

\begin{table}[]
    \centering
    \tiny
    \begin{tabular}{lccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{5}{c}{Korean} \\
    \cmidrule(lr){2-6}
                                      & MS    & R-1  & R-2  & R-L  & BLEU \\
    \midrule
    \textsc{LLaVA1.5 (13B)}           & 65.2  & 14.2 & 5.0  & 14.1 & 4.4 \\
    \midrule
    \textsc{KoLLaVA}                  & 66.0  & 20.6 & 8.1  & 20.5 & 4.1 \\       
    \midrule
    \textsc{X-LLaVA}                  & 59.6  & 15.7 & 5.5  & 15.8 & 12.2 \\
    %\textsc{X-LLaVA+Ours(En)}        & 62.8  & 25.9 & 25.8 & 13.3 \\
    \textsc{X-LLaVA+VLR-IF(Ko)}       & 63.6  & 24.3 & 9.7  & 24.0 & 13.2 \\
    \textsc{X-LLaVA+VLR-IF(En+Ko)}    & 62.4  & 25.2 & 10.1 & 25.2 & 12.2 \\       
    \bottomrule
    \end{tabular}
    \caption{Keyword matching korean}
    \label{tab:keyword_matching_ko}
\end{table}



==> table/no_ext_chinese_eval_table.tex <==
\begin{table}[]
    \tiny
    \centering
    \begin{tabular}{lcccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\vspace{-0.5em}Model}} & \multicolumn{4}{c}{Chinese}  \\
    \cmidrule(lr){2-5} & MS & ROUGE-1 & ROUGE-L & BLEU \\
    \midrule
    \textsc{QWEN-VL-CHAT}      & 13.6 & 8.1   & 0.8  & 0.0  \\
    \midrule
    \textsc{CHINESE-LLaVA}     & 7.6 & 5.1   & 0.1  & 5.0 \\
    \midrule
    \textsc{LLaVA1.5(13B)}     & 7.2 & 0.2   & 3.3  & 0.0 \\
    %\textsc{LLaVA1.5(13B)+Ours} & 50.8 & 27.3   & 27.2  & 1.2 \\
    \bottomrule
    \end{tabular}
    \caption{Keyword matching results on Chinese}
    \label{tab:no_ext_chinese}
\end{table}



==> table/no_ext_english_eval_table.tex <==
\begin{table}[]
    \centering
    \tiny
    \begin{tabular}{lccccc}
        \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{\vspace{-0.5em}Model}} & \multicolumn{5}{c}{English} \\
        \cmidrule(lr){2-6} 
                                   & MS & R-1 & R-2 & R-L & BLEU \\
        \midrule
        \textsc{BLIP-2}            & 6.4 & 22.8 & 6.4 & 22.3 & 0.0 \\
        \midrule
        \textsc{InstructBLIP}      & 0.8 & 6.2  & 1.6  & 5.7   & 4.5 \\
        \midrule
        %\textsc{LLaVA1.5 (7B)}     & 84.8 & 46.0   & 39.6 & 14.7  \\
        \textsc{LLaVA1.5 (13B)}    & 25.6 & 40.1 & 22.5 & 34.2 & 7.9  \\
        %\midrule
        %\textsc{Xtuner1.0}         & 84.0 & 47.0   & 41.1 & 13.8  \\
        \midrule
        \textsc{Xtuner1.1}         & 20.4 & 30.4 & 15.7 & 25.3 & 6.8  \\
        \midrule
        \textsc{X-LLaVA}           & 20.8 & 42.7 & 23.2 & 36.5 & 10.7 \\
        \midrule
        \textsc{Qwen-VL-Chat}      & 31.2 & 46.1 & 27.7 & 40.8 & 11.8 \\
        \midrule
        \textsc{GPT-4o}           & 61.6 & 68.5  & 49.5 & 63.5 & 33.7 \\
        \bottomrule
    \end{tabular}
    \caption{Keyword matching result english(no context)}
    \label{tab:no_ext_english}
\end{table}



==> table/no_ext_korean_eval_table.tex <==
% \begin{table}[]
%     \tiny
%     \begin{tabular}{c|cccc}
%     \toprule
%     \multicolumn{1}{c|}{\multirow{2}{*}{\vspace{-0.5em}Model}} & \multicolumn{4}{c|}{English} & \multicolumn{4}{c}{Korean} \\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%                                & MS & ROUGE-1 & ROUGE-L & BLEU \\
%     \midrule
%     \textsc{LLaVA1.5 (7B)}     & 80.0 & 25.0 & 24.7 & 5.4 \\
%     \textsc{LLaVA1.5 (13B)}    & 65.2   & 14.2  & 14.1 & 4.4 \\
%     \midrule
%     \textsc{KoLLaVA}           & 66.0 & 20.6 & 20.5 & 4.1 \\       
%     \midrule
%     \textsc{X-LLaVA}           & 59.6 & 15.7 & 15.8 & 12.2 \\
%     \textsc{X-LLaVA+Ours(En)}  & 62.8 & 25.9 & 25.8 & 13.3 \\
%     \textsc{X-LLaVA+Ours(En+Ko)}      & 62.4 & 25.2 & 25.2 & 12.2 \\       
%     \bottomrule
%     \end{tabular}
%     \caption{Keyword matching result}
%     \label{tab:korean_eval_table}
% \end{table}

\begin{table}[]
    \centering
    \tiny
    \begin{tabular}{lccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{5}{c}{Korean} \\
    \cmidrule(lr){2-6}
                               & MS  & R-1 & R-2  & R-L & BLEU \\
    \midrule
    \textsc{LLaVA1.5 (13B)}    & 2.4 & 3.5 & 0.8  & 3.4 & 2.3 \\
    \midrule
    \textsc{KoLLaVA}           & 5.2 & 1.9 & 0.0  & 1.9 & 0.7 \\       
    \midrule
    \textsc{X-LLaVA}           & 6.0 & 6.8 & 0.4  & 6.7 & 3.5 \\
    %\textsc{X-LLaVA+Ours(En)}  & 62.8 & 25.9 & 25.8 & 13.3 \\
    \bottomrule
    \end{tabular}
    \label{tab:no_ext_korean}
    \caption{Keyword matching korean(no context)}
\end{table}



==> table/performance_wrt_passage.tex <==
\begin{table}[h]
    \tiny
    \centering
    \begin{tabular}{llrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\vspace{-0.5em}Model}} & \multicolumn{6}{c}{English} \\
    \cmidrule(lr){2-7} 
    & PSG & MS & R-2 & R-L & BLEU & B-Score\\
    \midrule
    
    \textsc{LLaVA-LLaMA-3}   & GS  & 68.0 & 33.5 & 44.3 & 16.2 & 82.0 \\
                             & GB  & 59.6 & 30.4 & 40.9 & 14.6 & 81.0 \\
                             & SS  & 41.2 & 23.3 & 33.7 & 10.6 & 78.3 \\
                             & SB  & 38.4 & 23.4 & 33.5 & 10.4 & 78.3 \\
                             & B   & 22.4 & 19.5 & 29.6 & 09.2 & 76.4 \\
    \bottomrule
    \end{tabular}    
    % \caption{Xtuner's per-passage performance}
    \caption{Performance of \textsc{Llava-Llama-3} on Various Passages}
    \label{tab:performance_wrt_passage_xtuner}
\end{table}


==> table/quantitative_evaluation_0shot.tex <==
\begin{tabular}{lllllllll}
\toprule
 & $MMLU$ & H-swag & KOBEST & BOOLQ\textsuperscript{k} & COPA\textsuperscript{k} & H-swag\textsuperscript{k} & S-Neg\textsuperscript{k} & WIC\textsuperscript{k} \\
\midrule
$LLAMA8B(32,5)$ & $62.02$ & $60.16$ & $52.38$ & $50.57$ & $65.0$ & $42.6$ & $50.63$ & $\textbf{48.81}$ \\
$LLAMA8B^{F}(32,5)$ & $61.66$ & $\textbf{60.85}$ & $52.58$ & $50.36$ & $64.7$ & $42.0$ & $\textbf{55.16}$ & $\textbf{48.81}$ \\
$LLAMA8B^{L}(32,5)$ & $60.83$ & $60.69$ & $52.34$ & $50.14$ & $65.5$ & $42.4$ & $50.63$ & $\textbf{48.81}$ \\
$TARGET(32,5)$ & $58.87$ & $60.04$ & $51.7$ & $50.28$ & $60.7$ & $\textbf{42.8}$ & $54.41$ & $\textbf{48.81}$ \\
$EFT(32,5)$ & $\textbf{62.23}$ & $60.66$ & $52.53$ & $50.57$ & $\textbf{65.8}$ & $42.2$ & $51.13$ & $48.73$ \\
32layers_full & $25.49$ & $26.0$ & $46.26$ & $50.21$ & $46.6$ & $25.4$ & $49.62$ & $\textbf{48.81}$ \\
$EFT^{F}(32,5)$ & $62.02$ & $60.65$ & $52.36$ & $50.28$ & $65.1$ & $41.6$ & $52.39$ & $\textbf{48.81}$ \\
$EFT^{T}(32,5)$ & $54.44$ & $60.01$ & $51.13$ & $50.28$ & $62.2$ & $38.4$ & $49.62$ & $\textbf{48.81}$ \\
$EFT(32,20)$ & $62.09$ & $60.56$ & $52.47$ & $50.64$ & $\textbf{65.8}$ & $41.8$ & $50.63$ & $48.73$ \\
$EFT^{F}(34,5)$ & $57.53$ & $58.57$ & $50.69$ & $\textbf{51.42}$ & $56.1$ & $42.4$ & $50.88$ & $\textbf{48.81}$ \\
$EFT_{A}^{F}(34,5)$ & $62.07$ & $60.56$ & $\textbf{52.71}$ & $50.28$ & $65.4$ & $42.2$ & $54.91$ & $\textbf{48.81}$ \\
\bottomrule
\end{tabular}


==> table/quantitative_evaluation_5shot.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{4pt}
\begin{threeparttable}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
 &
  \multicolumn{4}{c|}{L2 (Learner)} &
  \multicolumn{4}{c|}{L1 (Native)} &
  \multicolumn{4}{c|}{Lang8} &
  \multicolumn{4}{c|}{Union (L1+L2)} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Gen.\\ time\end{tabular}}
  \\ \cline{2-17} &
  \multirow{2}{*}{GLEU} &
  \multicolumn{3}{c|}{$M^2$} &
  \multirow{2}{*}{GLEU} &
  \multicolumn{3}{c|}{$M^2$} &
  \multirow{2}{*}{GLEU} &
  \multicolumn{3}{c|}{$M^2$} &
  \multirow{2}{*}{GLEU} &
  \multicolumn{3}{c|}{$M^2$} &
  \\ \cline{3-5} \cline{7-9} \cline{11-13} \cline{15-17}
  & & Pre. & Rec. & $F_{0.5}$ & & Pre. & Rec. & $F_{0.5}$ & & Pre. & Rec. & $F_{0.5}$ & & Pre. & Rec. & $F_{0.5}$ &
   \\ \hline
\begin{tabular}[c]{@{}c@{}}Self-Scores\\[5pt] \end{tabular} &
  25.54 &
  1 &
  0 &
  0 &
  25.71 &
  1 &
  0 &
  0 &
  20.01 &
  1 &
  0 &
  0 &
  21.66 &
  1 &
  0 &
  0 &\\ 
\begin{tabular}[c]{@{}c@{}}Hanspell \\[5pt] \end{tabular} &
  30.36 &
  29.45 &
  5.33 &
  15.46 &
  57.08 &
  81.93 &
  47.36 &
  71.50 &
  22.94 &
  29.18 &
  8.74 &
  19.88 &
  28.82 &
  37.34 &
  11.58 &
  25.85 &
  189.69 \\ 
\begin{tabular}[c]{@{}c@{}}KoBART \\[5pt] \end{tabular} &
  45.06 &
  43.35 &
  24.54 &
  37.58 &
  67.24 &
  75.34 &
  55.95 &
  70.45 &
  28.48 &
  37.56 &
  11.62 &
  25.93 &
  33.70 &
  44.75 &
  14.64 &
  31.70 &
  38.25 \\ 
\midrule
\begin{tabular}[c]{@{}c@{}}\textsc{llama2-13B} \\[5pt] \end{tabular} &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  &
  &
  &
  & - \\ 

\begin{tabular}[c]{@{}c@{}}\textsc{llama3-8B-Inst(5shot)} \\[5pt] \end{tabular} &
  33.23 &
  26.33 &
  39.01 &
  24.45 &
  39.73 &
  32.65 &
  29.54 &
  31.98 &
  - &
  - &
  - &
  - &
  35.97&
  28.85&
  22.59&
  33.91& 
  63.24 \\
  
\begin{tabular}[c]{@{}c@{}}\textsc{llama3-8B-Inst+KAGAS} \\[5pt] \end{tabular} &
  52.35 &
  55.64 &
  37.22 &
  50.63 &
  82.18 &
  90.70 &
  78.66 &
  88.01 &
  - &
  - &
  - &
  - &
  62.73 &
  68.67 &
  50.24 &
  63.98& - \\ 

\begin{tabular}[c]{@{}c@{}}\textsc{KULLM+KAGAS} \\[5pt] \end{tabular} &
  56.71 &
  59.59 &
  44.29 &
  55.74 &
  83.17 &
  91.78 &
  80.01 &
  89.16 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - & - \\ 
  
\begin{tabular}[c]{@{}c@{}}\textsc{bllossom-novocab+KAGAS} \\[5pt] \end{tabular} &
  53.64 &
  58.93 &
  38.49 &
  53.22 &
  82.29 &
  92.13 &
  78.37 &
  89.01 &
  - &
  - &
  - &
  - &
  63.42 &
  72.08 &
  51.05 &
  66.59 & - \\ 
\begin{tabular}[c]{@{}c@{}}\textsc{bllossom-novocab+GEC+KAGAS} \\[5pt] \end{tabular} &
  54.65 & % 53.64
  60.33 & % 58.93
  40.66 & % 38.49
  55.01 & % 53.22 
  82.03 & % 82.29 
  92.05 & % 92.13
  78.05 & % 78.37
  88.87 & %89.01
  - &
  - &
  - &
  - &
  64.18 &
  71.58 &
  51.65 &
  66.45 & - \\ 
\begin{tabular}[c]{@{}c@{}}\textsc{bllossom-novocab+MUL+KAGAS} \\[5pt] \end{tabular} &
  54.21 & 
  59.30 & 
  39.78 & 
  54.00 &
  81.56 & 
  90.92 & 
  77.40 & 
  87.85 & 
  - &
  - &
  - &
  - &
  63.40 &
  70.94 &
  50.90 &
  65.76 & - \\ 
\begin{tabular}[c]{@{}c@{}}\textsc{bllossom-Inst-GEC} \\[5pt] \end{tabular} &
  36.54 &
  35.25 &
  20.47 &
  30.80 &
  40.12 &
  40.24 &
  35.56 &
  39.21 &
  - &
  - &
  - &
  - &
  37.51 &
  37.29 &
  25.33 &
  34.07 & 
  52.41 \\ 
  
\begin{tabular}[c]{@{}c@{}}\textsc{bllossom-KAGAS} \\[5pt] \end{tabular} &
  48.54 &
  52.99 &
  33.95 &
  47.64 &
  78.83 &
  86.02 &
  75.82 &
  83.76 &
  - &
  - &
  - &
  - &
  58.74 &
  67.26 &
  45.53 &
  61.40 & 
  52.41 \\ 

\begin{tabular}[c]{@{}c@{}}\textsc{bllossom-Inst-KAGAS} \\[5pt] \end{tabular} &
  47.13 &
  51.02 &
  32.69 &
  45.88 &
  78.16 &
  84.73 &
  75.15 &
  82.62 &
  - &
  - &
  - &
  - &
  58.62 &
  67.00 &
  45.16 &
  61.09 & 
  52.41 \\ 

\begin{tabular}[c]{@{}c@{}}\textsc{bllossom-Inst-GEC+KAGAS} \\[5pt] \end{tabular} &
  49.00 &
  53.46 &
  34.22 &
  48.05 &
  77.81 &
  84.81 &
  74.41 &
  82.51 &
  - &
  - &
  - &
  - &
  59.41 &
  67.97 &
  46.56 &
  62.24 &
  52.41 \\ 
  
\begin{tabular}[c]{@{}c@{}}\textsc{bllossomE-Inst-MUL+KAGAS} \end{tabular} &
  48.20 &
  53.00 &
  33.76 &
  47.57 &
  78.40 &
  85.67 &
  74.93 &
  83.28 &
  - &
  - &
  - &
  - &
  58.76 &
  67.17 &
  45.90 &
  61.47 & 
  52.41 \\ 
  \bottomrule
\end{tabular}}
\end{threeparttable}
\caption{\citeauthor{yoon-etal-2023-towards}가 제안한 GEC 데이터를 통한 실험결과. \textsc{bllossomE}는 본 연구에서 제안한 모델을 의미하며 \textsc{bllossomE+}는 GEC, AWE를 함께 학습한 멀티태스크 모델}
\label{tabs:experiments_gec}
\end{table*}




==> table/total_eval_table.tex <==

\begin{table*}[ht!]
\tiny
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\vspace{-0.5em}Model}} & \multicolumn{4}{c}{English} & \multicolumn{4}{c}{Korean} & \multicolumn{4}{c}{Chinese}\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
                           & MS & ROUGE-1 & ROUGE-L & BLEU & MS & ROUGE-1 & ROUGE-L & BLEU & MS & ROUGE-1 & ROUGE-L & BLEU \\
\midrule
\textsc{BLIP-2}             & 50.0 & 36.0 & 33.0 & 4.9  &  &  &  &   &  &  &  &  \\
\midrule
\textsc{InstructBLIP}       & 32.0 & 44.6 & 38.1 & 11.2 &  &  &  &  &  &  &  &  \\
\midrule
%\textsc{LLaVA1.5 (7B)}     & 84.8 & 46.0   & 39.6 & 14.7  \\
\textsc{LLaVA1.5 (13B)}     & 88.4 & 47.9   & 41.4 & 15.6 & 65.2 & 14.2   & 14.1 & 4.4 & 52.4 &  22.8   & 22.3  & 0.7 \\
%\midrule
\midrule
\textsc{KoLLaVA1.5}         &  &    &  &  & 66.0 & 20.6   & 20.5 & 4.1 &  &    &  &   \\
%\textsc{Xtuner1.0}         & 84.0 & 47.0   & 41.1 & 13.8  \\
\midrule
\textsc{Xtuner1.1}          & 79.2 & 48.5   & 42.8 & 15.4 &  &    &  &  &  &    &  & \\
\textsc{Xtuner1.1+Ours}     & 85.6 & 60.4   & 54.1 & 26.8 &  &    &  &  &  &    &  & \\
\midrule
\textsc{X-LLaVA}            & 80.4 & 54.3   & 47.2 & 20.2 & 59.6 &  15.7  & 15.8 & 12.2 &  -  &   -  &  -   &\\
\textsc{X-LLaVA+Ours(En)}   & 82.4 & 57.7   & 50.5 & 24.3 & -    &  -     & -    & -    &  -  &   -  &  -   &\\
\textsc{X-LLaVA+Ours(Ko)}  & 78.7  & 59.1  & 52.1 & 24.8 & 63.6 &  24.3  & 24.0 & 13.2 &\\
\textsc{X-LLaVA+Ours(En+Ko)}& 82.8 & 58.8   & 51.9 & 25.3 & 62.4 &  25.2  & 25.2 & 12.2 &  -  &   -  &  -   & \\
\midrule
\textsc{Qwen-VL}            & 85.4 & 61.5 & 55.9 & 25.0 &  &    &  &  & 51.6 & 25.0 & 25.0 & 1.1\\
\midrule
\textsc{CHINESE-LLAVA}      &  &  &  &  &  &    &  &  & 21.6 & 19.1 & 18.9 & 0.2\\
\midrule[0.8pt]
\textsc{GPT-4o}             & 88.8 & 64.5 & 59.2 & 29.5 &  &    &  &  &  &    &  & \\
\bottomrule
\end{tabular}
\caption{Keyword matching result english}
\label{tab:keyword_matching_total}
\end{table*}

==> table/total_experiments.tex <==
\begin{table*}
  \centering
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\"a}|     & {\"a}           \\
    \verb|{\^e}|     & {\^e}           \\
    \verb|{\`i}|     & {\`i}           \\
    \verb|{\.I}|     & {\.I}           \\
    \verb|{\o}|      & {\o}            \\
    \verb|{\'u}|     & {\'u}           \\
    \verb|{\aa}|     & {\aa}           \\\hline
  \end{tabular}
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\c c}|    & {\c c}          \\
    \verb|{\u g}|    & {\u g}          \\
    \verb|{\l}|      & {\l}            \\
    \verb|{\~n}|     & {\~n}           \\
    \verb|{\H o}|    & {\H o}          \\
    \verb|{\v r}|    & {\v r}          \\
    \verb|{\ss}|     & {\ss}           \\
    \hline
  \end{tabular}
  \caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
  \label{tab:total_experiments}
\end{table*}

